Class-Discriminative CNN Compression

Compressing convolutional neural networks (CNNs) by pruning and distillation has received ever-increasing focus in the community. In particular, designing a class-discrimination based approach would be desired as it fits seamlessly with the CNNs training objective. In this paper, we propose class-discriminative compression (CDC), which injects class discrimination in both pruning and distillation to facilitate the CNNs training goal. We first study the effectiveness of a group of discriminant functions for channel pruning, where we include well-known single-variate binary-class statistics like Student's T-Test in our study via an intuitive generalization. We then propose a novel layer-adaptive hierarchical pruning approach, where we use a coarse class discrimination scheme for early layers and a fine one for later layers. This method naturally accords with the fact that CNNs process coarse semantics in the early layers and extract fine concepts at the later. Moreover, we leverage discriminant component analysis (DCA) to distill knowledge of intermediate representations in a subspace with rich discriminative information, which enhances hidden layers' linear separability and classification accuracy of the student. Combining pruning and distillation, CDC is evaluated on CIFAR and ILSVRC 2012, where we consistently outperform the state-of-the-art results.

==> Supplementary_Material/model_details.tex <==
\section{Pruned Models Details}\label{sec:exp_details}


We show the detailed structures of our pruned VGG-16 and ResNet-50 on ILSVRC-2012 in Table~\ref{tab:VGG-16-Model} and~\ref{tab:ResNet-50-Model}. 
Both pruned models are named as \metric-B in the experimental results section.
On VGG-16, we find that our algorithm prunes more channels in shallow layers, 
which indicates the shallow layers are less sensitive to pruning than the deep ones under the same FLOPs reduction. 
On ResNet-50, our model preserves more channels at the starting blocks of each stage. 
These blocks have stride-2 downsampling connections,
which suggests that preserving information for the resolution reduction process would be crucial to maintain the network's performance.





